Uncertainty Annotated Databases - A Lightweight Approach for Approximating Certain Answers (extended version)

Certain answers are a principled method for coping with uncertainty that arises in many practical data management tasks. Unfortunately, this method is expensive and may exclude useful (if uncertain) answers. Thus, users frequently resort to less principled approaches to resolve the uncertainty. In this paper, we propose Uncertainty Annotated Databases (UA-DBs), which combine an under- and over-approximation of certain answers to achieve the reliability of certain answers, with the performance of a classical database system. Furthermore, in contrast to prior work on certain answers, UA-DBs achieve a higher utility by including some (explicitly marked) answers that are not certain. UA-DBs are based on incomplete K-relations, which we introduce to generalize the classical set-based notions of incomplete databases and certain answers to a much larger class of data models. Using an implementation of our approach, we demonstrate experimentally that it efficiently produces tight approximations of certain answers that are of high utility.

==> background-pdbs.tex <==
\subsection{Probablistic and Incomplete Data Models}
\label{sec:prob-data-models}

\BG{I think we should focus here on introducing the semantics and factor out the discussion of usability and move it somewhere else (maybe back to intro or later). I think the complexity results can be stated at the end (both TIs and PC-tables have \#P)}
% \OK{This section, while interesting, is not really necessary for this paper.  We show reductions from TI-PDBs and X-Tuples, not C-Tables or Tuple Bundle relations.  If we're going to get rid of something... this section would be a good candidate.}



The naive representation of PDBs as sets of possible world introduces redundancy by repeating tuples across many possible worlds. 
Hence, existing \abbrPQP systems rely on more compact encodings. 
% tuples sampled from different worlds are grouped together into tuple bundles $t$, or sparse arrays, with each element  each from a different sampled worlds.
% uses a tuple bundle model, where a tuple bundle $t$ is an array of tuples with same schema.
% The elements of this array ($t[i]$) are the value of
% $t$ in $i$th possible world. Example~\ref{example:mcdb} shows an tuples bundle
% representation of $PDB$ instance that can be derived from
% the PDB shown in Figure~\ref{table:pdb}.

\mypar{Tuple-Independent Databases}
A tuple independent probabilistic database (\abbrTI) $\pdb$ is a database instance where each tuple $\tup$ is annotated with its marginal probability $0<\probOf{\tup}\leq 1$. 
The probabilistic database represented by a \abbrTI $\pdb$ is the power-set of all of its tuples: For each tuple we decide whether the tuple should be part of the possible world or not. 
As the name indicates, in \abbrTI 's the existence of tuples is assumed to be independent of each other. 
Thus, the probability of a possible world $\db$ is the product of probabilities of tuples that do appear and one minus the probability of tuples that do not:
$$\probOf{\db} = \left(\prod_{\tup\in \db} \probOf{\tup}\right) \cdot \left(\prod_{\tup \not \in \db} 1 - \probOf{\tup}\right)$$

\mypar{(P)C-Tables}
\textit{C-Tables}~\cite{DBLP:journals/jacm/ImielinskiL84} enrich the active domain of the database with an set $\Sigma$ of variable symbols, sometimes called labeled nulls or skolem terms, which are used to represent unknown values.
The set of possible worlds defined by a C-table $\pdb$ is the set of instances that are derived from $\pdb$ by replacing each variable symbol from $\Sigma$ according to a valuation $v$ which assigns variables to constants from $\aDom$.
Allowable valuations may be restricted by defining a global condition, a boolean expression over symbols from $\Sigma$ that a valuation must satisfy.
Finally, tuples are annotated by a local condition,  a boolean expression over comparison of values from $\Sigma \cup \aDom$.  
The tuple appears only in worlds where the local condition is satisfied.
When the global condition is replaced by a joint probability distribution over allowable valuations, the resulting structure is called a Probabilistic-, or PC-Table~\cite{DBLP:journals/debu/GreenT06}.
Both C-Tables and PC-Tables are closed under relational algebra, and can be extended for closure under generalized projection~\cite{5447879} and aggregation~\cite{Green:2007:OFC:1247480.1247631}. C-tables generalize several other incomplete database models. For instance, a \textit{V-table} is a C-table without local and global conditions (all conditions are constant true) and a \textit{Codd-table} is a V-table where no variable appears more than once.

\BG{aS discussed we may remove tuple bundles:}
% \mypar{Tuple Bundles}
% Although PC-Tables provide a lossless encoding of the set of possible worlds, these encodings are not generally intended for human consumption.
% Rather, it is typical to present query outputs using the marginal distribution, or confidence, for each output tuple.
% Computing marginals over PC-Tables is \texttt{\#P}-complete in general~\cite{DS07b,suciu2011probabilistic}, making approximations~\cite{DBLP:journals/vldb/FinkHO13} necessary. 
% As a result some systems like MCDB~\cite{jampani2008mcdb} instead adopt a data model based that uses sampling from the start.
% In this strategy, probabilistic data is encoded as a finite collection of samples drawn from the set of possible worlds. 
% Queries are then evaluated over these samples in parallel, producing a collection of results sampled from the possible results of the query.
% To make query evaluation efficient, MCDB uses structures called tuple-bundles that encode the value of the same tuple across different samples.  
% Attributes that are identical across all samples are stored as primitives, while attributes that vary are stored as arrays.
% Finally, a bit-vector is used to indicate which samples the tuple-bundle appears in.

% enrich the relational model with variables. A tuple in a c-table consists of constants and variables.
% Each assignment of the variables present in a c-table corresponds to one possible world represented by the c-table. Furthermore, each tuple in a c-table is associated with a boolean condition $\phi$ over the c-table's variables. A tuple is part of a possible world corresponding to a variable assignment if its condition evaluates to true for this assignment. A pc-table extends c-tables by recording a probability distribution for each variable. 
% interpret all possible values for a
% variable as a separate table.
% Example~\ref{example:c-table} shows an instance of
% table~\ref{table:pdb} in c-table representation.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[t]
% \centering
%   \begin{tabular}{ c|c|cc }
%     % \cline{1-3}
%     \textbf{name}  & \textbf{color}  & \textbf{category} & \underline{\textbf{isPres}}  \\
%     \cline{1-3}
%     apple & red & fruit & [T,T,T]\\
    
%     apple & green & fruit & [T,T,T]\\
    
%     carrot & red & vegetable & [T,T,T]\\
    
%     tomato & red & [fruit,vegetable,fruit] & [T,F,T]\\
%     % \cline{1-3}
%   \end{tabular}
% \bfcaption{Tuple bundles representing $\query_{fru}(\pdb)$.}
% \label{table:mcdb}
% \end{figure}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \centering
  \begin{tabular}{ c|c|cc }
  \textbf{name}  & \textbf{color}  & \textbf{category} & \underline{\textbf{$\prob$}}  \\
    \cline{1-3}
    apple & red & fruit & 1\\
    
    apple & green & fruit & 1\\
    
    tomato & red & fruit & 0.6\\
      \end{tabular}
  \bfcaption{\abbrTI representing the query result $\query_{fru}(\pdb)$}
  \label{fig:ti-example-query-result}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example} \label{example:mcdb}
  % Figure~\ref{table:mcdb} shows an example tuple bundle representation of 3 samples ($\db_1, \db_2, \db_1$) taken from the possible results $\query(\pdb)$ shown in Figure~\ref{table:pqp}.
  % Tuple bundles are annotated with a bit vector indicating which samples the bundle contributes a tuple to (e.g., the tuple for tomatoes does not appear in sample 2).
  % Attribute values that vary by sample are stored as arrays.
% \end{Example}
% \begin{Example}
  % \label{example:c-table}
% In pc-tables, possible worlds are expressed by introducing variables to individual attributes. Each variable is associated with a probability distribution.
  Figure~\ref{table:c-table} shows a pc-table representation of the same query result. 
  Uncertainty about the category of tomatoes is encoded using a variable $x_1$ with the probability distribution as shown in the figure.
  \BG{Explain figure~\ref{fig:ti-example-query-result}}
\end{Example}

\begin{figure}[t]
  \centering
  \begin{subtable}{.7\linewidth}\label{table:c-table-table}
  \centering
  \begin{tabular}{ c|c|cl }
    % \cline{1-3}
    \textbf{name} & \textbf{color}  & \textbf{category} & \underline{$\phi$} \\
    \cline{1-3}&&&\\[-3.1mm]
    apple & red & fruit & T \\
    
    apple & green & fruit & T\\
     
    carrot & red & vegetable & T\\
    
    tomato & red & \redL{$x_1$} & $\redL{x_1} = \text{`fruit'}$\\
    % \cline{1-3}
  \end{tabular}
  \vspace*{-1mm}
  \caption{C-table}
  \end{subtable}
  
  \begin{subtable}{.5\linewidth}\label{table:c-table-probdist}
      \centering
      \begin{align*}
        x_1 &= 
        \begin{cases}
          \text{fruit}  &0.6\\
          \text{vegetable} & 0.4\\
        \end{cases}
      \end{align*}
  % \begin{tabular}{ |c|c|c| }
  %   \hline
  %   \textbf{variable}  & \textbf{value}  & \textbf{P}  \\
  %   \hline
  %   $x_1$ & fruit & 0.6 \\
    
  %   $x_1$ & vegetable & 0.4\\
  %   \hline
  % \end{tabular}
  \vspace*{-2mm}
      \caption{Probability Distribution}
  \end{subtable}
\bfcaption{PC-Table representing $\query(\pdb)$.} % With another table storing probability distributions for all variables.}
\label{table:c-table}
\end{figure}

Query evaluation over queries in this form is in \texttt{\#P} in general. 
One class of approaches exploit that certain queries are in \texttt{PTIME}~\cite{DBLP:journals/vldb/FinkHO13,DBLP:conf/vldb/AgrawalBSHNSW06}, approximate probabilities~\cite{4221832,5447879}, or compute only relative rankings~\cite{DBLP:journals/vldb/GatterbauerS17,DBLP:journals/vldb/LiSD11}.




==> introduction-Jan24-uarelations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{UA-relations}
\label{sec:ua-relations}


\mypar{Bag Semantics}
An important advantage of our approach is that it also supports bag semantics. This in particular relevant if we apply UA-relations for an approach such as Mimir that introduces uncertainty as part of queries over deterministic data, because the input relation would be stored in a relational database which uses bag semantics.% , thus, may contain duplicates.
\BG{The previous sentence needs to be written better}. 

\begin{Example}\label{example:bag-UA-relation-UAA-relation}
  Reconsider possible worlds representation of the probabilistic database $\pdb$ from Figure~\ref{table:pdb} and uncertainty taint representation derived from $\pdb$ in Figure~\ref{table:example-UT}. Figure~\ref{table:example-UA} shows the UA-relation representation of the same uncertainty taint approach while adapting bag semantics where tuples are annotated by natural numbers recording the multiplicity of the tuple. In UA-relation, we use a pair of numbers to record the multiplicity of a tuple and multiplicity of certain respectively. i.e. (1,1) denotes the tuple repeats 0 times uncertain and 1 time certain. 
%  We further extend the UA-relation to UAA-relation that is shown in Figure~\ref{table:example-UAA}. An attribute value is marked certain if the value is the same in all possible worlds were the tuple exists. 
  We have developed a technique that uses conventional query processing to produce the UA-result for a query if applied to the UA-relational representation of a PDB without requiring conventional \abbrPQP to be applied. % as shown in Example~\ref{example:pqp}
\end{Example}



%As shown in Example~\ref{example:UT}, instead of using a full probabilistic database, we only consider the instance from the probabilistic database with the highest probability and mark tuples and attribute values as either certain or uncertain. Intuitively, a tuple is tainted as certain if the tuple exists in all instances of the probabilistic database and tainted as uncertain if the tuple only exists in some of the instances.


%An attribute in a tuple is tainted as certain if the value is the same in all instances of the probabilistic database where the tuple exists and tainted uncertain otherwise. 
Obviously, the UA-database corresponding to a possible world of a PDB does not retain all the information encoded by the PDB, e.g., the UA-database does not record probabilities and does not encode information about tuples that do not occur in the possible world the UA-database corresponds to.  However, the advantage of UA-relations is that query evaluation is significantly more efficient than query evaluation over probabilistic databases. We propose and implement a query rewriting approach that evaluates queries over UA-relations by propagating uncertainty taints. This approach has performance that is close to deterministic query processing. Herein lies the main advantage of UA-relations, as a non-destructive approximation of uncertainty that allows for fast query evaluation. Figure~\ref{fig:overview} shows an overview of our approach. We assume that probabilistic databases stores in some model are given. Alternatively, we can apply our approach in the context of a system like Mimir~\cite{Yang:2015:LOA:2824032.2824055} which introduces uncertainty on the fly. 
%\BG{explain correctness criteria.}

\begin{figure}[t]
  \centering
  \begin{subtable}{\linewidth}
  \centering
  \caption{$\pdb$ in uncertainty taint representation}
  \begin{tabular}{ |c|c|c|l }
        \cline{1-3}
    \textbf{name}  & \textbf{color}  & \textbf{category}  & \\
    \cline{1-3}
    apple & red & fruit & \tcMarker\\
        
    pear & yellow & fruit& \tcMarker\\
        
    carrot & red & vegetable& \tcMarker\\
        
    tomato & red & fruit& \tuMarker\\
        \cline{1-3}
  \end{tabular}
  \label{table:example-UT}
  \end{subtable}
  
  \begin{subtable}{\linewidth}
  \centering
  \caption{UA-relation bag representation}
  \begin{tabular}{ |c|c|c|l }
        \cline{1-3}
    \textbf{name}  & \textbf{color}  & \textbf{category}  & \\
    \cline{1-3}
    apple & red & fruit & (1,1)\\
        
    pear & yellow & fruit& (1,1)\\
        
    carrot & red & vegetable& (1,1)\\
        
    tomato & red & fruit& (1,0)\\
        \cline{1-3}
  \end{tabular}
  \label{table:example-UA}
  \end{subtable}
  
% \begin{subtable}{\linewidth}
% \centering
% \caption{UAA-relation bag representation}
% \begin{tabular}{ |c|c|c|l }
%       \cline{1-3}
%   \textbf{name}  & \textbf{color}  & \textbf{category}  & \\
%   \cline{1-3}
%   \cMarker{apple} & \cMarker{red} & \cMarker{fruit} & (1,1)\\
%       
%   \cMarker{pear} & \cMarker{yellow} & \cMarker{fruit} & (1,1)\\
%       
%   \cMarker{carrot} & \cMarker{red} & \cMarker{vegetable} & (1,1)\\
%       
%   \cMarker{tomato} & \cMarker{red} & \uMarker{fruit} & (1,1)\\
%       \cline{1-3}
% \end{tabular}
% \label{table:example-UAA}
% \end{subtable}
  
\caption{Uncertainty marker representation: use the possible world with the highest probability and mark attributes and tuples as either $T$=certain or $\redL{F}$=uncertain. For bag semantics representation, we annotate tuples with a pair of values representing the total multiplicity of the tuple and certain duplicates of this tuple, respectively.}
\label{table:UT-rep}
\end{figure}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
  \centering
  
% \begin{subtable}{\linewidth}
  \centering
% \caption{Query over bag UA-relation}
  \begin{tabular}{ |c|l }
        \cline{1-1}
    \textbf{category}  & \\
    \cline{1-1}
    fruit & (3,2)\\
                
    vegetable & (1,1)\\
    \cline{1-1}
  \end{tabular}
% \label{table:example-UA-res}
% \end{subtable}
  
% \begin{subtable}{\linewidth}
% \centering
% \caption{Query over bag UAA-relation}
% \begin{tabular}{ |c|l }
%       \cline{1-1}
%   \textbf{category}  & \\
%   \cline{1-1}
%   \cMarker{fruit} & (2,2)\\
%       
%   \cMarker{vegetable} & (1,1)\\
%       
%   \uMarker{fruit} & (1,1)\\
%       \cline{1-1}
% \end{tabular}
% \label{table:example-UAA-res}
% \end{subtable}
  \caption{Query evaluation over uncertainty-annotated relations}
  \label{fig:qp-over-ua-relations}
\end{figure}
%%%%%%%%%%%%%%%%%%%%

==> introduction-Jan24-uncertaintyannotations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Uncertainty Annotations}
\label{sec:uncertainty-labeling}
\BG{This subsection needs to be organized better. We need to explain separately set and bag semantics as well as UAA and we need examples for query evaluation.}
\BG{Maybe introduce uncertainty labelings first or not???}

In this paper, we study light-weight representations of uncertainty which enrich the data of one possible world from a probabilistic database with uncertainty information. Specifically, we study relations where tuples (and possibly attribute values) are annotated with uncertainty labels (certain or uncertain). Given a probabilistic database $\pdb$, we can derive an uncertainty-annotated database (\abbrUADB) by annotating the tuples in one possible world $\db \in \pdb$ (typically the possible world with the highest probability) with uncertainty labels. Given an \abbrUADB $\uadb$ for a possible world $\db$ of a \abbrPDB $\pdb$ we say the database is \textit{c-sound} if every tuple marked as certain is certain in $\pdb$. Similar an $\uadb$ is called \textit{c-complete} if all certain tuples of $\pdb$ are marked as certain. Note that for most probabilistic data models it is trivial to derive a c-sound and c-complete UA-database.

The query semantics we define for \abbrUADBs is backward compatible to deterministic processing. That is, ignoring annotations, the result of a query over a \abbrUADB is the same as evaluating the same query over the possible world from which we have derived the \abbrUADB.
Furthermore,  the result of a query is c-sound as long as the input is c-sound, i.e., we never label a tuple as certain in a query result if the tuple is not a certain answer to the query according to the input \abbrPDB. However, query answers only guaranteed to be c-complete for certain classes of queries. We argue that declaring an uncertain result as certain is more objectionable than declaring a certain result as uncertain. Thus, c-soundness is more important than c-completeness. \BG{remove that if we do not demonstrate it}
Note that given the complexity of exact \abbrCAQP we cannot hope for an efficient query evaluation algorithm that preserves both both c-sound and c-complete. 
In summary, our approach combines the advantages of best guess query processing with approximation of certain answer semantics: 1) query evaluation is efficient and can be expressed in SQL, 2) all certain answers to the query will be returns, 3) the labelling of an answers determines whether the answer is certain or not. 

\begin{Example}\label{example:UT}
%\BG{say something about c-soundness/perservation}
  Reconsider the \abbrPDB from Figure~\ref{table:pdb}, Figure~\ref{table:example-UT} shows a set semantics uncertainty labeling derived from the running example possible world $\db_1$ (the possible world with the highest probability). Note that the labeling is c-sound (and c-complete) and we can always derive c-sound uncertainty taint from an instance of \abbrPDB  \BG{Give this relation a name for query evaluation}
To generate this representation, we annotate each tuple in the possible world as either certain ($\tcMarker$) or uncertain ($\tuMarker$). A row is marked certain if the row exists in all possible worlds of the probabilistic database and as uncertain otherwise. In this example, only the last tuple (red tomato) is uncertain and, thus, is annotated with $\tuMarker$. Now consider the evaluation of a query $\query_{cat} = \projection_{category}(\db)$ from Example~\ref{example:pqp} over this encoding. The results are shown in Figure~\ref{fig:qp-over-ua-relations}. Both result tuples are certain, since there exists a certain tuple with these category values.
\end{Example}


% The purpose of this exercise is to enable fast query evaluation over uncertain data which pairs the advantages of deterministic query processing (efficiency and ease of use) with certain answer semantics (

In this paper, we introduce UA-relations (Uncertainty Annotated-relations), relations where tuples are annotated with uncertainty taints. We employ UA-relations as a low-overhead representation of probabilistic data that allows queries to be evaluated efficiently. Given a probabilistic database $\pdb$, we can derive an UA-database by annotating the tuples in one possible world $\db \in \pdb$ (typically the possible world with the highest probability) with uncertainty taints that capture information about the presence of the tuple in $\pdb$. 
%To deal effectively with probabilistic data models that use attribute-level uncertainty (e.g., pc-tables), we extend UA-databases by also annotating attribute values with uncertainty taints - we call the resulting model \textit{UAA-relations} (Uncertainty Annotated Attribute databases).
We study query evaluation over such relations and demonstrate that two important correctness properties hold:
1) ignoring annotations, the result of a query over a UA-relation is the same as evaluating the same query over the possible world from which we have created the UA-relation and 2) we never label a tuple as certain in a query result if the tuple is not a certain answer to the query according to the input \abbrPDB. \BG{The result is that we get the best of both worlds: deterministic query evaluation, but still keeping important uncertainty information}




When evaluating queries over possible world annotated with uncertainty labels, we expect the query results to be annotated in a way that is consistent with the result of the conventional query processing without labeling and the labeling can provide extra uncertainty information to the user.

==> labelschemes.tex <==
\input{introduction-Jan24-uncertaintyannotations.tex}


Recall that our goal is to annotate tuples from one possible world with uncertainty information and then design a query semantics over such annotated data which propagates uncertainty in a way that is compatible with possible world query semantics. For this we define a class of semirings whose elements are pairs of values from $\kDom$, i.e., elements from $\dpK{\semK}{2}$. Such a pair $(d,c)$ will be used to record the annotation $d$ that the tuple carries in the possible world as well as the part $c$ of the annotation  that is certain.  Given an annotation $k = (d,c)$ we define:

\begin{align}
  \cOf{k} &= c & \dOf{k} &= d
\end{align}
%$\cOf{k} = c$ and $\uOf{k} = u$.

% \begin{Definition}[Uncertainty Label Semirings]
% For any a m-semiring  $\semK$, we define a semiring $\uK = (\uKDom, \addOf{\uK}, \multOf{\uK}, \zeroOf{\uK}, \oneOf{\uK})$ where $\uKDom = \kDom^2$ and the operations are defined pointwise based on the corresponding operations for $\pwK$.
% \end{Definition}

We now define uncertainty labelings of a possible world $\db$ as $\dpK{\semK}{2}$-databases where the $\dOf{k}$ component of a tuple $\tup$'s annotation is equal to $\db(\tup)$.  % that replace the annotations in a possible world with annotations from $\uK$.

\section{Uncertainty Labelings}
\label{sec:uncert-labell}
\BG{We need examples in this section, probably more clear explanations, definition for bag AUL needs to be checked for correctness. Also the macros $\backslash TUL$ and $\backslash AUL$ are ugly, let's come up with a better notation}
We now introduce labeling schemes that enrich a possible world from a probabilistic database with uncertainty information by annotating tuples (and potentially also attribute values) as either certain or uncertain. We then proceed to define intuitive correctness criteria for such labelings. We define labelling for both set and bag semantics probabilistic databases. For instance, we should not label tuples as certain that are not certain in the probabilistic database from which the labelling stems from. To be able to label attribute values we start by introduce domains of values that are either labelled as certain ($\tcMarker$) or uncertain ($\tuMarker$). Furthermore, we define matching of tuples with such values, a relaxed version of equality which ignore uncertain attribute values.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Labelled Domain and Tuple Matching]
  Consider a universal domain $\aDom$ of values. Given a set of uncertainty labels $\uLabels = \{\tcMarker, \tuMarker\}$, we define $\uDom = \{ d^{l} \mid l \in \uLabels \wedge d \in \aDom\}$, the labelled version of $\uDom$. Given a labelled value $d^{l}$ we define an operator $\labelOf$ the extracts the label from the value: $\labelOf(d^{l}) = l$.   Given a tuple $\tup = (\aVal_1, \ldots, \aVal_n)$ and $\tup_{\uLabels} = (e_1, \ldots, e_n)$ such that $\aVal_i \in \aDom$ and $e_i \in \uDom$ we say $t$ matches $\tup_{\uLabels}$, written as $\tup \tmatches \tup_{\uLabels}$ if for all $i \in \{1, \ldots,n\}$ either $\labelOf(e_i) = \tcMarker$ or $\aVal_i = e_i$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For instance, a tuple $(1,3)$ would match a tuple $(\uMarker{2}, \cMarker{3})$, but not a tuple $(\cMarker{2}, \uMarker{3})$. Given a relation $\rel$ we define $\ltupDom(\rel)$ the set of labelled tuples with the same schema as $\rel$ ($\ltupDom(\db)$ is defined analog).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Set Semantics Labelings}
\label{sec:set-semant-labell}

We define tuple and attribute-level uncertainty labelings. Tuple labelings are simplify functions that map every tuple from a $\tupDom(\db)$ to a value from $\uLabels$ or the special value $\notHere$ to indicate that the tuple does not belong to $\db$. While we could alternatively just map tuples from $\db$ instead of using $\tupDom(\db)$ and the additional label $\notHere$, using total functions enables us to define sets and bags in an analog fashion.
For attribute-level uncertainty labelings, we define labelled versions of databases and relations where each attribute value is marked as either certain or uncertain.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{Definition}[Attribute-labelled Database]
%   Consider a database $\db$ over a domain $\aDom$. We say a database $\ldb$ over $\uDom$ with the same schema s $\db$ is an attribute-labelling of $\db$ iff the condition shown below holds. We define labelings of relations in the same fashion.
%   \begin{align*}
%     \forall \tup \in \db: \exists \tup' \in \ldb: \tup \tmatches \tup' \wedge (\forall \tup'' \in \ldb: \tup \tmatches \tup'' \rightarrow \tup' = \tup'')\\
%     \forall \tup \in \ldb: \exists \tup' \in \db: \tup' \tmatches \tup \wedge (\forall \tup'' \in \db: \tup'' \tmatches \tup' \rightarrow \tup' = \tup'')
%   \end{align*}
% \end{Definition}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Uncertainty Labeling]
  Let $\pdb$ be a probabilistic database and $\db$ one of its possible worlds. A tuple uncertainty labeling $\TUL$ for the pair $(\pdb,\db)$ is a function from $\tupDom(\db)$ to $\{ \tcMarker, \tuMarker, \notHere \}$ such that for all $\tup \in \tupDom(\db)$ we have $\TUL(\tup) = \notHere \Leftrightarrow \tup \not\in \db$. An attribute uncertainty labeling  $\AUL$ for the pair $(\pdb,\db)$ is a function $\ltupDom(\db) \mapsto \{\tcMarker, \tuMarker, \notHere \}$ such that:
  \begin{itemize}
  \item $\forall \tup \in \tupDom(\db): t \in \db \Leftrightarrow \exists \tup' \in \ltupDom(\db): \tup \tmatches \tup' \wedge \AUL(\tup') \neq \notHere$
   \item $\not\exists \tup \in \tupDom(\db), \tup_1, \tup_2 \in \ltupDom(\db): \tup \tmatches \tup_1 \wedge \tup \tmatches \tup_2 \wedge \AUL(\tup_1) \neq \notHere \wedge \AUL(\tup_2) \neq \notHere$
  \end{itemize}
  % \begin{align}
  %   \forall \tup \in \db: \exists \tup' \in \ltupDom(\db): \tup \tmatches \tup' \wedge \AUL(\tup') \neq \notHere \wedge (\forall \tup'' \in \ltupDom(\db): \AUL(\tup'') = \notHere \vee (\tup \tmatches \tup'' \rightarrow \tup' = \tup''))\\
  %   \forall \tup \in \ldb: \exists \tup' \in \db: \tup' \tmatches \tup \wedge (\forall \tup'' \in \db: \tup'' \tmatches \tup' \rightarrow \tup' = \tup'')
  % \end{align}
  % a tuple labeling $\TUL$ for $(\pdb, \db)$ and a function $\AUL$ from each attribute value (pair of tuple and attribute) to $\{ \tcMarker, \utMarker \}$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Intuitively, the definition of attribute labelings ensures that only one labelled version of each tuple in $\db$ is mapped to a label different from $\notHere$. Furthermore, only labelled versions of tuples which do not exist have to be mapped to $\notHere$. Note that an attribute labeling maps each tuple $\tup \in \db$ to exactly one labelled tuple, the only labeled version of $\tup$ which is not mapped to $\notHere$. In the following use $\tup_{\AUL}$ to denote the labelled tuple assigned to
$\tup$ by an attribute uncertainty labeling $\AUL$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Example}
  Reconsider

  \BG{Reexplain (part of) an intro example given the formalism}
\end{Example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness Criteria for Set Labelings}
\label{sec:corr-crit-sets}

Of course, a labeling should assign the $\tcMarker$ and $\tuMarker$ annotations in a way that is coherent with the input probabilistic database $\pdb$. Ideally, a tuple uncertainty labeling (TUL) should assign the $\tcMarker$ label only to tuples that are certain (exist in all possible worlds of $\pdb$) and assigns the $\tuMarker$ label to all other tuples. However, as we will see there is a trade-off between the computational complexity of generating such a labeling and maintaining it under queries and fulfilling this correctness criterion. Thus, we also introduce less strict correctness criteria to not have to sacrifice efficiency. For an attribute uncertainty labeling, we have to define what we mean by a tuple $\tup$ with  uncertain attribute values to occur in a possible world since the tuple may have different values in different possible worlds.
\BG{needs examples}
% For that we define tuple matchings. For an AUL $\AUL$ for $(\pdb,\db)$, a labeled tuple $\tup_l$ matches a tuple $\tup$ from a possible $\db \in \pdb$, written as $\tup_l \tmatches \tup$, if $\tup$ agrees with $\tup_l$ on all certain attribute values (where $\AUL(\tup_l, A)= \tcMarker$).
\BG{Discuss why c-soundness is more critical then c-completeness (either here or already in intro}
\BG{@move this to related work? Explain relationship to m-tables labelings to make clear the relationship and distinction}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[C-soundness and C-completeness]
  Let $\pdb$ be a probabilistic database and $\db$ one of its possible worlds. A TUL $\TUL$ is
  \begin{itemize}
  \item \textbf{c-sound} if $\forall \tup \in \db: \TUL(\tup) = \tcMarker \Rightarrow \tup \in \cSet(\pdb)$
  \item \textbf{c-complete} if $\forall \tup \in \db: \tup \in \cSet(\pdb) \Rightarrow \TUL(\tup) = \tcMarker$
  \end{itemize}
  Analog, an AUL $\AUL$ is

  \begin{itemize}
  \item \textbf{c-sound} if
    $\forall \tup \in \db: \TUL(\tup) = \tcMarker \Rightarrow \forall \db' \in
    \pdb: \exists \tup' \in \db': \tup \tmatches \tup'$

    \item   \textbf{c-complete} if $\forall \db' \in \pdb: \exists \tup' \in \db': \tup \tmatches \tup' \Rightarrow \TUL(\tup) = \tcMarker$

\end{itemize}

\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BG{define tuple matching between two labelled tuples too, so far does not look like we need that.}

Additionally, since we want to be able to evaluate queries over a labeling we have to require that (1) ignoring labels, queries behave exactly like deterministic queries over $\db$ and (2) that queries preserve the correctness of a labeling. For instance, if the labeled input of a query $\query$ is both c-sound and c-complete, then the output query $\query$ evaluated over this input should be c-sound and c-complete wrt. the full probabilistic query result ($\query(\pdb)$). We call this property preservation of c-soundness/c-completeness under queries.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Preservation of Correctness under Queries]
Let $\TUL$ be a c-sound/c-complete TUL for $(\pdb,\db)$ and $\query$ a query from a class of queries $\qClass$. A semantics for evaluating queries over labelling is said to preserve c-soundness/c-completeness if for $\query(\TUL)$ is a c-sound/c-complete labeling for $(\query(\pdb), \query(\db))$. The definition of AUL is analog.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Note that if a query semantics for a labeling scheme preserves both c-soundness and c-completeness, then it follows that it behaves like deterministic query evaluation for deterministic inputs (a PDB with one possible world). However, since the UA- and UAA-relations we introduce are only c-sound for some classes of queries, we are interested in this additional correctness criteria which we will refer to as \textit{backward compatibility} (with deterministic query semantics).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bag Semantics Labelings}
\label{sec:bag-semant-label}



Furthermore, since we also target bag semantics, we extend the notions of a tuple uncertainty labeling and attribute uncertainty labeling as well as correctness criteria for bag instances.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}[Bag Labeling]
  Given a probabilistic database $\pdb$ with bag semantics and one of its possible worlds $\db$, a TUL $\TUL$ for $(\pdb, \db)$ is a function that assigns to each tuple $\tup \in \db$ a pair of natural numbers $(u,c) \in \semN \times \semN$ with $|(u,c)| = u + c = \db(\tup)$. Given a tuple $\tup = (a_1, \ldots, a_n)$, a labelled version of tuple $\tup$ is a tuple $\tup_l = ({a_1}^{l_1}, \ldots, {a_n}^{l_n})$ where each $l_i \in \{\tcMarker, \tuMarker\}$.
  An AUL for $(\pdb,\db)$ is a function whose input is the set of all labelled tuples for tuples from $\db$ and whose domain is $\semN \times \semN$. Note that AUL may split $\tup$ into set of $\tup_l$s as $S$ such that $\db(t) = \sum_{\tup_l \in S}|TUL(\tup_l)|$.
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\BG{Do we have a better way of defining bag AULs?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Correctness Criteria for Bag Labelings}
\label{sec:corr-crit-sets}


The pair of natural numbers $(u,c)$ assigned by a bag TUL to a tuple denotes the tuple's certain and uncertain multiplicity. That is, $u + c$ is the multiplicity of $\tup$ in $\db$ and ideally $c = \cMult(\pdb,\tup)$. For a bag AUL, multiple annotated we record certain and uncertain multiplicities for each possible combination of attribute labels for a tuple. Based on these versions of TULs and AULs for bag semantics PDBs, we now define c-soundness and c-correctness (preservation of correctness is the same for set and bag semantics).
To define these properties for bag AULs, We define a global tuples matching function $GM$ maps a triple of the form $(\tup_l,\db,\tup)$ to a natural number $n$ where $\db \in \pdb$ and $\tup \in \db$ and $\tup_l \tmatches \tup$ and $\tup_l \in \db_l$. Here $\db_l$ denotes group of all labeled tuples. The function means a labeled tuple $\tup_l$ is matched to $n$ multiplicities of tuples $\tup \in D$. For a global tuple matching $GM$, define restrictions:
$$\forall \db \in \pdb: \forall \tup \in \db: \db(t) \geq \sum_{\tup_l \in \db_l}GM(\tup_l,\db,\tup) $$
$$\forall \db \in \pdb: \forall \tup_l \in D_l: |TUL(\tup_l)| \geq \sum_{\tup \in \db}GM(\tup_l,\db,\tup) $$
The first restriction enforces that each duplicate of tuple $\tup$ can match to at most one labeled tuple $\tup_l$. The second restriction enforces that a labeled tuple can not match to number of tuples more than its own multiplicity. Then we extend $\cMult$ to take matching into account:
\begin{align}
	\cMatches(GM,\pdb,\tup_l)=\min_{\db \in \pdb}(\sum_{\tup \in \db}GM(\tup_l,\db,\tup))
\end{align}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Definition}
  Let $\pdb$ be a bag probabilistic database and $\db$ one of its possible worlds. Let $\TUL(\tup) = (u,c)$. We use $c_\tup$ denote $c$ for a given tuple $\tup$. A TUL $\TUL$ is
  \begin{itemize}
  \item \textbf{c-sound} if $\forall \tup \in \db: c_\tup \leq \cMult(\pdb, \tup)$
  \item \textbf{c-complete} if $\forall \tup \in \db: c_\tup \geq \cMult(\pdb, \tup)$
  \end{itemize}
  Analog, an AUL $(\TUL,\AUL)$ is

  \begin{itemize}
  \item \textbf{c-sound} if \\
    $\exists GM: \forall \tup \in \db: c_t \leq \cMatches(GM,\pdb,\tup) $
  \item   \textbf{c-complete} if \\
  	$\exists GM: \forall \tup \in \db: c_t \geq \cMatches(GM,\pdb,\tup) $
    \end{itemize}
\end{Definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{Example} \label{example:labeltup}
Consider a c-sound UA-relation tuple (apple,red,fruit) with annotation $(1,2)$. The annotation indicates there are three duplicate tuples in the single possible world we labeling on, and all possible worlds have at least one duplicate of this tuple. Consider a c-sound UAA-relation tuple (\cMarker{apple},\uMarker{red},\cMarker{fruit}) with annotation $(1,2)$. The annotation indicates there are three duplicate tuples of (apple,red,fruit) in the single possible world we labeling on, and all possible worlds have at least one duplicate of tuple can uniquely match to (apple,*,fruit) where * can be any value.
%  \BG{Show for a single tuple some labelled tuples with different multiplicities and discuss what this means.}
\end{Example}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uadb"
%%% End:


==> querysem.tex <==
\section{Query Semantics}
\label{sec:rules}
\SF{Updated}
\BG{This needs more context in the beginning to make clear the connection and difference with K-relational query semantics}

In this section, We introduce propagation and rewriting rules on top of the uncertainty model in both tuple and attribute level. We start with apply our annotation semiring $K_{uncert}$ to standard K-relation querying semantics on applicable relation algebra operators. Then we extend the querying semantics to UAA-relations where, different from traditional K-relations model, attribute level annotations and row level annotations are both involved. At last we state some non-monotone relational algebra operators that can not be properly defined by K-relational models and discuss how to properly query our them while preserving c-soundness. Let $rowD(Q,t,I)$ denote the row determinism for tuple $t$ in the result of query $Q$ over database instance $I$. Let $attrD(Q,t,A,I)$ denote the determinism for attribute $A$ of tuple $t$ in the result of query $Q$ over instance $I$.
%Let $exprD(t,E)$ denote the determinism for expression $E$ of tuple $t$. If a row is marked as certain then it belongs to the set of certain answers which also called c-sound. If it is marked uncertain then it may belong to the set of certain answers or may be uncertain which means c-completeness is not guaranteed.%


\subsection{UAA-relation query semantics}
UAA-relations maintain similar querying semantics on projection, cross product and union operations. For positive queries, attribute level uncertainty is maintained in the output because the uncertainty is embedded in the universe itself. So the attribute determinism is trivially $attrD(Q,t,A,I)=det(t.A)$. For selection and join operation with clauses, attribute level annotations may propagate to row level annotations. In this case, we may need to map attribute level determinism to row level annotation structure because some query operators determine row based on attribute values. Define transfer function that transfer an boolean expression $\theta$ into row level annotations:
\[
trans(\theta(t))=\begin{cases}
    (0,1), & \text{if } [[\theta((t))]]=T^T\\
    (1,0), & \text{if } [[\theta((t))]]=T^F\\
    (0,0), & \text{else}
\end{cases}
\]

Then specify modified selection and join querying semantics as:
\begin{enumerate}

\item selection
\[rowD(\selection_\theta(Q),t,I)=rowD(Q,t,I) \otimes trans(\theta(t))\]

\item join
\begin{align*}
	rowD(Q_1 & \join_\theta Q_2,t,I) \\
	=&rowD(Q_1,t,I) \otimes rowD(Q_2,t,I) \otimes trans(\theta(t))
\end{align*}

\end{enumerate}

Join and selection involves row level uncertainty affected by attribute level uncertainty using  function $trans()$ that transfer a annotated expression evaluation result into row level taint structure. Projection may involving grouping of same tuples leading to addition operation similar to union. Example \ref{example:attr-full} shows a fully annotated database instance and the step-by-step propagated result by the propagation rules.


\begin{Example}
	Figure~\ref{table:4.full} shows a full detailed example by executing query \\
	$\projection_{color}(\selection_{color='red'}(food \join_{category=pref} preference))$ over a UAA-relation instance \textsf(food) and \textsf(preference). First join operator outputs first and third tuple with row annotations $(1,3) \otimes (0,2)=(2,6)$ and $(2,1) \otimes (0,2)=(4,2)$ respectively. Second tuple row level annotation is calculated as $(0,2)\otimes(1,1)\otimes(1,0)=(4,0)$ since $ [[vegetable^T=vegetable^F]]=T^F $. Second operator as selection only changes row annotation of third tuple into $(4,2)\otimes(1,0)=(6,0)$ since $ [[red^F=[['red']]]]=[[red^F=red^T]]=T^F $. Third operator as projection sums up identical tuples giving second result tuple row annotation to be $(4,0)\oplus(6,0)=(10,0)$.
\label{example:attr-full}
\end{Example}

\begin{figure}[ht]
	\centering
	\begin{subtable}{\linewidth}
	\centering
	\caption{Tainted input table: \textsf{food}}
	\begin{tabular}{ |c|c|c|l}
				\cline{1-3}
		\textbf{name}  & \textbf{color}  & \textbf{category}   & \\
		\cline{1-3}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} & (1,3)\\
%				\cline{1-3}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} & (0,2)\\
%				\cline{1-3}
		\cMarker{apple} & \uMarker{red} & \cMarker{fruit} & (2,1)\\
				\cline{1-3}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Tainted input table: \textsf{preference}}
	\begin{tabular}{ |c|c|l}
				\cline{1-2}
		\textbf{group}  & \textbf{pref}   & \\
		\cline{1-2}
		\cMarker{child} & \cMarker{fruit} & (0,2)\\
%				\cline{1-2}
		\cMarker{adult} & \uMarker{vegetable} & (1,1)\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Join result}
	\begin{tabular}{ |c|c|c|c|c|l}
				\cline{1-5}
		\textbf{name}  & \textbf{color}  & \textbf{category} & \textbf{group}  & \textbf{pref}  & \\
		\cline{1-5}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (2,6)\\
%				\cline{1-5}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} & \cMarker{adult} & \uMarker{vegetable} & (4,0)\\
%				\cline{1-5}
		\cMarker{tomato} & \uMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (4,2)\\
				\cline{1-5}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Selection result}
	\begin{tabular}{ |c|c|c|c|c|l}
				\cline{1-5}
		\textbf{name}  & \textbf{color}  & \textbf{category} & \textbf{group} & \textbf{pref}  & \\
		\cline{1-5}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (2,6)\\
%				\cline{1-5}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} & \cMarker{adult} & \uMarker{vegetable} & (4,0)\\
%				\cline{1-5}
		\cMarker{tomato} & \uMarker{red} & \cMarker{fruit} & \cMarker{child} & \cMarker{fruit} & (6,0)\\
				\cline{1-5}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{final result after projection}
	\begin{tabular}{ |c|l}
				\cline{1-1}
		\textbf{color}  &\\
		\cline{1-1}
		\cMarker{red} & (2,6)\\
%				\cline{1-1}
		\uMarker{red} & (10,0)\\
				\cline{1-1}
	\end{tabular}
	\end{subtable}

\caption{A query execution with annotation propagation example on UAA-relation. (a)-(b) are input tables. (c)-(e) are intermediate and final output results.(current rule is not c-sound in case of multiple group by attributes)}
\label{table:4.full}
\end{figure}

\subsection{Non-monotone Queries}
There are several relational algebra operators involving negative operations which are not directly defined by our semiring model. Since we only propagating one possible world from the probabilistic database, in general cases input tuples may be filtered out un-deterministically by operations like selection over attributes containing uncertain data. Which means some tuples exist in partial worlds of conventional probabilistic query processing may missing in result of our model. For the current implementation, we are tainting all affected fields to uncertain to preserve c-sound property. We need to redefine grouping mechanism in aggregation operator for our model to work under the promise as well.\\
For the query evaluation for aggregation, we need to change grouping mechanism so that tuples are not grouped by their value in $\mathcal(U)^+$, but are grouped by the non-annotated value $val(v)$. i.e. for an input instance $R$ to the aggregation operator, we evaluate the value output for aggregation by first strip off all attribute level annotations. Then we reassign annotations to the output. Define function $strip_{all}(R)= \forall_{t \in R} : strip(t)$, Aggregation operator evaluation scheme is: $[[_g\gamma_F(R)]]=_g\gamma_F(strip_{all}(R))$. \\
Define function that map an annotation $(u,c)$ to its unit form as:
\[unit(u,c)=\begin{cases}
	(0,1), & \text{if } c>0 \\
	(1,0), & \text{if } c=0 \text{ and } u>0 \\
	(0,0), & \text{else}
\end{cases}
\]
Row level propagation rule is defined as:
\[rowD(_g\gamma_F(Q),t,I) = unit(\sum_{t'.g=t.g}rowD(Q,t',I))\]
Attribute level annotations for group by attributes are picked from one of the tuples $t'$ from the group where $rowD(_g\gamma_F(Q),t,I)=unit(rowD(Q,t',I))$. The naive heuristic is to pick a tuple with most number of certain group by attributes. Without completeness information, aggregation result attributes are annotated with uncertain so that c-sound hold in aggregation operators.\\
Similar situation happens in set difference operator where we need to set all output row level determinism to uncertain since we do not know if the input is complete. One way to optimize this issue and potentially produce less conservative result by sacrificing performance is to propagating extra information in the rewriting recording weather the input of a operator contain tuples that are conditionally eliminated (p-completeness).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uadb"
%%% End:


==> uaa-correctness.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Expression Evaluation over $\mathcal{U}^+$ is c-sound]
\label{theo:expr-c-sound}
  Let $\pdb$ be a probabilistic database and $\db$ be a c-sound UAA-database wrt. $\pdb$, then for any tuple $t \in \db$, and some expression $e$. If $det([[ e(t) ]]) = T$, then in every possible world $D_i \in \pdb$ there has to exist a tuple $t'$ with $t \tmatches t'$ such that $[[e(t')]] = val([[e(t)]])$. % evaluates to the same result in every possible world.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
	We prove this theorem using induction over the structure of a expression under the assumption that the input to the expression is c-sound.

	\proofpara{Base case}
	When the expression is only a single attribute value $e=A.t$, output is c-sound following from the c-soundness assumption that we made for the input.

	\proofpara{Induction step} \\
	For expression operator $op(arg_1,arg_2,\ldots, arg_n)$, \\assume $arg_1(t),arg_2(t),\ldots, arg_n(t)$ is c-sound.
	\begin{itemize}
		\item CASE 1: For $op=\{+,-,=,>,<,||\}$ operations $op(l,r)$, the result is certain only if both of the input is certain $det(l(t))=det(r(t))=T$. Given $l(t)$ and $r(t)$ are c-sound which means $l(t)$ and $r(t)$ return same value for all $D_i \in \pdb$ where exist $t' \in D_i$ st. $t \tmatches t'$. So $op(l,r)(t)$ also returns same value for all $D_i \in \pdb$ where $t$ matching exist. So these operations are c-sound.
		\item CASE 2: For $op=\{*\}$ operation $op(l,r)$, the result is certain only if both of the input is certain or one of the value is $0^T$, $det(l(t))=det(r(t))=T \vee l(t)=0^T \vee r(t)=0^T$. Case $det(l(t))=det(r(t))=T$ is same as CASE 1 so under this case the operator is c-sound. For case $l(t)=0^T \vee r(t)=0^T$, we know either $r(t)$ or $l(t)$ is $0$ for all $D_i \in \pdb$ where exist $t' \in D_i$ st. $t \tmatches t'$. So $l*r=0$ for all $D_i \in \pdb$ where matching $t$ exists. So case $l(t)=0^T \vee r(t)=0^T$ is c-sound and overall the operator is c-sound.
		\item CASE 3: For $op={\wedge}$ operation $op(l,r)$, the result is certain iff both the input is certain or one of the value is $F^T$, $det(l(t))=det(r(t))=T \vee l(t)=F^T \vee r(t)=F^T$. Similar to CASE 2 where in this case we have $l \wedge F=F \wedge r=F$ for all $D_i \in \pdb$ where matching $t$ exists. So the operator is c-sound.
		\item CASE 4: For $op=\{\vee\}$ operation $op(l,r)$, the result is certain iff both the input is certain or one of the value is $T^T$, $det(l(t))=det(r(t))=T \vee l(t)=T^T \vee r(t)=T^T$. Similar to CASE 2 where in this case we have $l \vee T=T \vee r=T$ for all $D_i \in \pdb$ where matching $t$ exists. So the operator is c-sound.
		\item CASE 5: For $op=\{if\}$ operation $op(arg_{if},arg_{then},arg_{else})$, the result is certain iff the if condition is certain and corresponding consequence value is certain according to the condition, $ arg_{if}(t)=T^T \wedge det(arg_{then}(t))=T \vee (\neg arg_{if})(t)=T^T \wedge det(arg_{else}(t))=T$. For the case $arg_{if}(t)=T^T \wedge det(arg_{then}(t))=T$, by assumption we know $arg_{then}(t)$ is c-sound which means $arg_{then}(t)$ returns same value for all $D_i \in \pdb$ where exist $t' \in D_i$ st. $t \tmatches t'$. So $arg_{then}(t)$ itself as the output is c-sound. Same logic apply to case of $arg_{else}(t)$. So the operator is c-sound.
	\end{itemize}
	So by induction, we conclude that our expression evaluation model is c-sound by the fact that any expression is recursively start with the base case which is c-sound, and all the operator result is c-sound given the input is c-sound.
\end{proof}

Based on this result, we now proceed to prove that query evaluation preserves c-soundness, i.e., if the input to a query is c-sound wrt. a probabilistic database $\pdb$ then so is the output wrt. evaluating the query over $\pdb$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Query Evaluation Preserves c-Soundness in UAA-relation]\label{theo:UAA-are-c-sound}
  Let $\pdb$ be a probabilistic database and $\db$ be a UAA-database corresponding to $\pdb$ that is c-sound. Given a query $\query$, the result $\query(\db)$ is c-sound wrt. $\query(\pdb)$.
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
  We prove this theorem using induction over the structure of a query under the assumption that the input to the query is c-sound.

  \proofpara{Base case}
  When the query $\query$ is of the form $\query=R$, i.e., it consists of a single relation access, then c-soundness of the output following from the c-soundness assumption that we have made for the input.

\proofpara{Induction step} Assume that the query is of the form $op(\query_1)$ for some operator $op$ and assume that the result $\query_1$ is c-sound.
	\begin{itemize}
		\item For union operation $Q_1 \cup Q_2$, the result tuple $t$ with annotation $(u,c)$ is produced by adding annotation $(u_1,c_1)$ of $t' \in Q_1$ and annotation $(u_2,c_2)$ of $t' \in Q_2$ where $t'\tmatches t$ so that $c=c_1+c_2$. By assumption we know $Q_1(t')$ and $Q_2(t')$ is c-sound which means $c_1 \leqslant c_1^*$ and $c_2 \leqslant c_2^*$. By propagation rule we have $c=c_1+c_2 \leqslant c_1^*+c_2^*=c^*$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
		\item For join operation $Q_1 \times Q_2$, the result tuple $t$ with annotation $(u,c)$ is produced by multiplying annotation $(u_1,c_1)$ of $t_1 \tmatches t[SCHEMA(Q_1)] \in Q_1$ and annotation $(u_2,c_2)$ of $t_2 \tmatches t[SCHEMA(Q_1)] \in Q_2$ so that $c=c_1 \times c_2$. By assumption we know $t_1$ and $t_2$ are c-sound which means $c_1 \leqslant c_1^*$ and $c_2 \leqslant c_2^*$. By propagation rule we have $c=c_1 \times c_2 \leqslant c_1^* \times c_2^*=c^*$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
		\item For projection operation $\projection_{U}(Q)$, the result tuple $t$ with annotation $(u,c)$ is produced by adding all tuples $t_i$ with annotation $(u_i,c_i)$ respectively where $t_i \in Q \wedge t_i[U] \tmatches t$. By assumption we know all $t_i$s are c-sound which means $\forall_{i}(c_i \leqslant c_i^*)$. By propagation rule we have $c=\sum_{i}(c_i)<\sum_{i}(c_i^*)=c^*$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
		\item For selection operation $\selection_{\theta}(Q)$, the result tuple $t$ with annotation $(u,c)$ has $c>0$ iff $t \models \theta$. By assumption we know $Q(t')$ where $t' \tmatches t$ with annotation $(u_o,c_o)$ is c-sound which means $c_o \leqslant c_o^*$. By propagation rule we have $c=c_o<c_o^*=c^* \vee c=0$. So for all result possible worlds there exist at least $c$ repetitions of $t$, thus the result is c-sound.
	\end{itemize}
	So by induction, we conclude that our query rewriting rules is c-sound by the fact that any operator is recursively start with the base case which is c-sound, and all the operator result is c-sound given the input is c-sound.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uadb"
%%% End:


==> uaa-rels.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{UAA-Relations}\label{sec:uaa-model}
\SF{Updated}
\BG{This needs to be better structured and motivated. First give overview: we define annotationed domain U+ and define expression evaluation for this domain, then we create UA-relations over this new domain which we call UAA-relations}

We extend UA-relations model into UAA-relations (Uncertainty Attribute Annotated relations) by annotating each attribute in a tuple with a single binary value, define attribute determinism as a mapping between an attribute A from a tuple t and a binary(boolean) value: $\{F,T\}$ where label $F$ as uncertain and $T$ as certain.

\begin{Definition}[UAA-relations domain]
	For universe $\mathcal{U}$ as UA-relations domain, define UAA-relations domain to be universe $\mathcal{U}^+=\{v^T \mid v \in \mathcal{U}\} \cup \{v^F \mid v \in \mathcal{U}\} \cup \{T^T,T^F,F^T,F^F\}$ correspondingly.
\end{Definition}

The backward mapping from $\mathcal{U}^+$ to $\mathcal{U}$ is trivial by removing annotations from all values from $\mathcal{U}^+$. For any $v \in \mathcal{U}$ and $b \in \{T,F\}$, an tuple $t=<v_1^{b_1}, \ldots, v_n^{b_n}>$ from $\mathcal{U}^+$ value and annotation component from a UAA-relation domain can be processed seperatelly.
\begin{align}
  \label{eq:2}
  val(v^b) &= v\\
  det(v^b) &=b \\
  strip(t) &=<val(v_1^{b_1}), \ldots, val(v_n^{b_n})>
\end{align}
% $val(v^b)=v \mid v^b \in \mathcal{U}^+$.\\
%  $det(v^b)=b \mid v^b \in \mathcal{U}^+$.\\
%  $strip(t)=<val(v_1^{b_1}), \ldots, val(v_n^{b_n})> \mid t=<v_1^{b_1}, \ldots, v_n^{b_n}>$.\\
The annotation indicates the determinism of corresponding value in $\mathcal{U}$: \\$attrD(Q,t,A,I)=det(v^b) \mid t.A=v^b$.\\
Let $[[e]]$ denote the evaluation of a expression $e$ over values: $<v_1,v_2, \ldots, v_n> \in  \mathcal{U}^+$ or $<v_1,v_2, \ldots, v_n> \in  \mathcal{U}$. Assuming attribute annotated using semiring $(\{T,F\}, F, T, \vee, \wedge)$ and evaluation output of boolean expression over $\mathcal{U}^+$ to be in $\{T^T,T^F,F^T,F^F\}$, define each expression operator over $\mathcal{U}^+$ as following:
\begin{enumerate}
	\item arithmetic operators\\
	\[[[v_1^{b_1} \pm v_2^{b_2}]]=[[v_1 \pm v_2]]^{[[b_1 \wedge b_2]]}\]
	\[
	[[v_1^{b_1} \times v_2^{b_2}]]=\begin{cases}
	0^T, & \text{if} \; v_1=0^T \vee v_2=0^T\\
    [[v_1 \times v_2]]^{[[b_1 \wedge b_2]]}, & \text{else}
	\end{cases}
  \] \\
    \item comparison operators\\
	\[[[v_1^{b_1} = v_2^{b_2}]]=[[v_1 = v_2]]^{[[b_1 \wedge b_2]]}\]
	\[[[v_1^{b_1} > v_2^{b_2}]]=[[v_1 > v_2]]^{[[b_1 \wedge b_2]]}\]
	\[[[v_1^{b_1} < v_2^{b_2}]]=[[v_1 < v_2]]^{[[b_1 \wedge b_2]]}\]
	\item boolean operators\\
	\[[[\neg v_1^{b_1}]]=[[\neg v_1]]^{b_1}\]
	\[[[v_1^{b_1} \wedge v_2^{b_2}]]=[[v_1 \wedge v_2]]^{[[(\neg v_1 \wedge b_1) \vee (\neg v_2 \wedge b_2) \vee (b_1 \wedge b_2)]]}\]
	\[[[v_1^{b_1} \vee v_2^{b_2}]]=[[v_1 \vee v_2]]^{[[(v_1 \wedge b_1) \vee (v_2 \wedge b_2) \vee (b_1 \wedge b_2)]]}\]
	\item conditional operators\\
	\begin{align*}
		[[\text{if } v_1^{b_1} \text{ then } & v_2^{b_2} \text{ else } v_3^{b_3}]] \\
		& =[[\text{if } v_1 \text{ then } v_2 \text{ else } v_3]]^{[[(v_1 \wedge b_1 \wedge b_2) \vee (\neg v_1 \wedge b_1 \wedge b_3)]]}
	\end{align*}
	\item string operators\\
	\[[[v_1^{b_1} || v_2^{b_2}]]=[[v_1 || v_2]]^{[[b_1 \wedge b_2]]}\]
\end{enumerate}
Define expression determinism to be: \\
$exprD(t,E)=det([[E(t)]])$.\\

For the expression definitions above, string operator and most of the mathematical operators are straight forward that one uncertain value will make the result uncertain, beside multiplication with $0^T$ value will result $0^T$ independent of the other input value. In some boolean expressions, the output annotations will be depend on the value and the annotation of the input. Example \ref{example:expr-rule} shows briefly how the rules work in an database instance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Theorem}[Expression processing in $\mathcal{U}$ is embedded in $\mathcal{U^+}$]
Define transfer function $tr(v)=v^T \mid v \in \mathcal{U} \wedge v^T \in \mathcal{U^+}$. Define function $tr_{all}$ that apply $tr()$ to all values in expression $E$. then for any expression $E$, $tr_{all}([[E]])=[[tr_{all}(E)]]$.
\label{theo:expr-emb}
\end{Theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
We prove this theorem using induction over the structure of a expression.

	\proofpara{Base case} When $E$ is a single value, by assumption we know $[[v]]^T=[[v^T]]=v^T$.\\

	\proofpara{Induction cases} for each operator, we have
	\begin{align*}
		& [[v_1^T \pm v_2^T]] = v_1^T \pm v_2^T=(v_1 \pm v_2)^{T\wedge T}=[[(v_1 \pm v_2)]]^T\\
		& [[v_1^T \times v_2^T]]=(v_1 \times v_2)^{T \times T} = [[v_1 \times v_2]]^T \\
		& [[v_1^T (=,>,<) v_2^T]]=(v_1 (=,>,<) v_2)^{T} = [[v_1 (=,>,<) v_2]]^T \\
		&
		\begin{aligned}
    	[[v_1^T \wedge v_2^T]]= & (v_1 \wedge v_2)^{((v_1 \wedge v_2) \wedge T)\vee((v_1 \wedge v_2) \wedge T)\vee(T \wedge T)} \\
    	 = & (v_1 \wedge v_2)^T = [[v_1 \wedge v_2]]^T
    	\end{aligned} \\
    	&
    	\begin{aligned}
    	[[v_1^T \vee v_2^T]]= & (v_1 \vee v_2)^{((v_1 \vee v_2) \wedge T)\vee((v_1 \vee v_2) \wedge T)\vee(T \wedge T)} \\
    	= & (v_1 \vee v_2)^T = [[v_1 \vee v_2]]^T
    	\end{aligned} \\
    	&
    	\begin{aligned}
    		[[\text{if } v_1^T & \text{ then } v_2^T \text{ else } v_3^T]] \\
    		&=(\text{if } v_1 \text{ then } v_2 \text{ else } v_3)^{(v_1 \wedge T \wedge T) \vee (\neg v_1 \wedge T \wedge T)} \\
    		&=(\text{if } v_1 \text{ then } v_2 \text{ else } v_3)^T = [[\text{if } v_1 \text{ then } v_2 \text{ else } v_3]]^T\\
    	\end{aligned}
	\end{align*}
   	Thus by induction, for any operator, $T$ annotated input will result $T$ annotated output with value same as non-annotated operator result. So for any expression $E$, normal expression computation is embedded in our annotated model.
\end{proof}

\begin{Example}
	Table \ref{table:4.attr} shows an example instance of executing query
	$$Q=\projection_{name,color||\textvisiblespace^T||category}(food)$$.
	For the tuple $apple^T$, The value $red^T||\textvisiblespace^T$ is computed according to the rule return $red\textvisiblespace^{T \wedge T=T}$ and further combined with $fruit^T$ return the final tuple. For the tuple $carrot^T$, the first concatenation result is formed by $red^F||\textvisiblespace^T=red\textvisiblespace^{T \wedge F=F}$ and second concatenation produces $red\textvisiblespace vegetable^{F \wedge T=F}$ as the tuple result. The last tuple follows identical procedure with $F \wedge F=F$ for the last concatenation.
\label{example:expr-rule}
\end{Example}

\begin{figure}[t]
	\centering
	\begin{subtable}{\linewidth}
	\centering
	\caption{Tainted input table: \textsf{food}}
	\begin{tabular}{ |c|c|c|}
				\cline{1-3}
		\textbf{name}  & \textbf{color}  & \textbf{category}   \\
		\cline{1-3}
		\cMarker{apple} & \cMarker{red} & \cMarker{fruit} \\
%				\cline{1-3}
		\cMarker{carrot} & \uMarker{red} & \cMarker{vegetable} \\
%				\cline{1-3}
		\cMarker{tomato} & \uMarker{red} & \uMarker{fruit} \\
				\cline{1-3}
	\end{tabular}
	\end{subtable}

	\begin{subtable}{\linewidth}
	\centering
	\caption{Query result}
	\begin{tabular}{ |c|c| }
				\cline{1-2}
		\textbf{name} & \textbf{description} \\
				\cline{1-2}
		\cMarker{apple} & \cMarker{red fruit}\\
%				\cline{1-2}
		\cMarker{carrot} & \uMarker{red vegetable}\\
%				\cline{1-2}
		\cMarker{tomato} & \uMarker{red fruit}\\
				\cline{1-2}
	\end{tabular}
	\end{subtable}
\caption{expression combination rules example: result string is uncertain if any of the input strings are uncertain. The result is certain if all of the input strings are certain.}
\label{table:4.attr}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "uadb"
%%% End:

